Simultaneous Estimation and Group Identification for Network Vector Autoregressive Model with Heterogeneous Nodes

Individuals or companies in a large social or financial network often display rather heterogeneous behaviors for various reasons. In this work, we propose a network vector autoregressive model with a latent group structure to model heterogeneous dynamic patterns observed from network nodes, for which group-wise network effects and timeinvariant fixed-effects can be naturally incorporated. In our framework, the model parameters and network node memberships can be simultaneously estimated by minimizing a least-squares type objective function. In particular, our theoretical investigation allows the number of latent groups G to be over-specified when achieving the estimation consistency of the model parameters and group memberships, which significantly improves the robustness of the proposed approach. When G is correctly specified, valid statistical inference can be made for model parameters based on the asymptotic normality of the estimators. A data-driven criterion is developed to consistently identify the true group number for practical use. Extensive simulation studies and two real data examples are used to demonstrate the effectiveness of the proposed methodology.

==> macros/algorithm.tex <==


% \usepackage{algorithm,algorithmicx,algpseudocode}
% http://shantoroy.com/latex/how-to-write-algorithm-in-latex/
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}} % require \usepackage{xcolor}
\SetCommentSty{mycommfont}

\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output

==> macros/box-theorems.tex <==
% more info here
% https://texblog.org/2015/09/30/fancy-boxes-for-theorem-lemma-and-proof-with-mdframed/

\usepackage[framemethod=TikZ]{mdframed} % box environment & flexible box designs

% or
\usepackage{fancybox}

==> macros/self-defined.tex <==
% Copy right @ 2019
% All right reserved by Elynn Y. Chen.
% This file defines short-hands for math formulas.
% It started with  Prof. Jianqing Fan's macro definition.
% Later it incorporated some of my own macro definition.
%
%
% Other references:
% -- math guide: http://mirrors.rit.edu/CTAN/info/short-math-guide/short-math-guide.pdf
% -- bold math symbol: https://tex.stackexchange.com/questions/595/how-can-i-get-bold-math-symbols
%
%


\renewcommand{\bar}{\overline}
\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}

%--------------------------------
%
%  Boldfaces in Letters
%
% \newcommand{\bfm}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\bfm}[1]{\ensuremath{\boldsymbol{#1}}} % bm

\def\bzero{\bfm 0}
\def\bone{\bfm 1}
\def\bbone{\mathbbm{1}} % package bm

\def\ba{\bfm a}   \def\bA{\bfm A}  %\def\AA{\mathbb{A}}
\def\bb{\bfm b}   \def\bB{\bfm B}  \def\BB{\mathbb{B}}
\def\bc{\bfm c}   \def\bC{\bfm C}  \def\CC{\mathbb{C}}
\def\bd{\bfm d}   \def\bD{\bfm D}  \def\DD{\mathbb{D}}
\def\be{\bfm e}   \def\bE{\bfm E}  \def\EE{\mathbb{E}}
\def\bff{\bfm f}  \def\bF{\bfm F}  \def\FF{\mathbb{F}}
\def\bg{\bfm g}   \def\bG{\bfm G}  \def\GG{\mathbb{G}}
\def\bh{\bfm h}   \def\bH{\bfm H}  \def\HH{\mathbb{H}}
\def\bi{\bfm i}   \def\bI{\bfm I}  \def\II{\mathbb{I}}
\def\bj{\bfm j}   \def\bJ{\bfm J}  \def\JJ{\mathbb{J}}
\def\bk{\bfm k}   \def\bK{\bfm K}  \def\KK{\mathbb{K}}
\def\bl{\bfm l}   \def\bL{\bfm L}  \def\LL{\mathbb{L}}
\def\bm{\bfm m}   \def\bM{\bfm M}  \def\MM{\mathbb{M}}
\def\bn{\bfm n}   \def\bN{\bfm N}  \def\NN{\mathbb{N}}
\def\bo{\bfm o}   \def\bO{\bfm O}  \def\OO{\mathbb{O}}
\def\bp{\bfm p}   \def\bP{\bfm P}  \def\PP{\mathbb{P}}
\def\bq{\bfm q}   \def\bQ{\bfm Q}  \def\QQ{\mathbb{Q}}
\def\br{\bfm r}   \def\bR{\bfm R}  \def\RR{\mathbb{R}}
\def\bs{\bfm s}   \def\bS{\bfm S}  \def\SS{\mathbb{S}}
\def\bt{\bfm t}   \def\bT{\bfm T}  \def\TT{\mathbb{T}}
\def\bu{\bfm u}   \def\bU{\bfm U}  \def\UU{\mathbb{U}}
\def\bv{\bfm v}   \def\bV{\bfm V}  \def\VV{\mathbb{V}}
\def\bw{\bfm w}   \def\bW{\bfm W}  \def\WW{\mathbb{W}}
\def\bx{\bfm x}   \def\bX{\bfm X}  \def\XX{\mathbb{X}}
\def\by{\bfm y}   \def\bY{\bfm Y}  \def\YY{\mathbb{Y}}
\def\bz{\bfm z}   \def\bZ{\bfm Z}  \def\ZZ{\mathbb{Z}}
\def\vec{\mbox{vec}}
\def\wh{\widehat}
\def\ol{\overline}
\def\cor{\mbox{cor}}

\def\calA{{\cal  A}} \def\cA{{\cal  A}}
\def\calB{{\cal  B}} \def\cB{{\cal  B}}
\def\calC{{\cal  C}} \def\cC{{\cal  C}}
\def\calD{{\cal  D}} \def\cD{{\cal  D}}
\def\calE{{\cal  E}} \def\cE{{\cal  E}}
\def\calF{{\cal  F}} \def\cF{{\cal  F}}
\def\calG{{\cal  G}} \def\cG{{\cal  G}}
\def\calH{{\cal  H}} \def\cH{{\cal  H}}
\def\calI{{\cal  I}} \def\cI{{\cal  I}}
\def\calJ{{\cal  J}} \def\cJ{{\cal  J}}
\def\calK{{\cal  K}} \def\cK{{\cal  K}}
\def\calL{{\cal  L}} \def\cL{{\cal  L}}
\def\calM{{\cal  M}} \def\cM{{\cal  M}}
\def\calN{{\cal  N}} \def\cN{{\cal  N}}
\def\calO{{\cal  O}} \def\cO{{\cal  O}}
\def\calP{{\cal  P}} \def\cP{{\cal  P}}
\def\calQ{{\cal  Q}} \def\cQ{{\cal  Q}}
\def\calR{{\cal  R}} \def\cR{{\cal  R}}
\def\calS{{\cal  S}} \def\cS{{\cal  S}}
\def\calT{{\cal  T}} \def\cT{{\cal  T}}
\def\calU{{\cal  U}} \def\cU{{\cal  U}}
\def\calV{{\cal  V}} \def\cV{{\cal  V}}
\def\calW{{\cal  W}} \def\cW{{\cal  W}}
\def\calX{{\cal  X}} \def\cX{{\cal  X}}
\def\calY{{\cal  Y}} \def\cY{{\cal  Y}}
\def\calZ{{\cal  Z}} \def\cZ{{\cal  Z}}


%--------------------------------
%
%  Boldfaces in Greek
%
\newcommand{\bfsym}[1]{\ensuremath{\boldsymbol{#1}}}

 \def\balpha{\bfsym \alpha}
 \def\bbeta{\bfsym \beta}
 \def\bgamma{\bfsym \gamma}             \def\bGamma{\bfsym \Gamma}
 \def\bdelta{\bfsym {\delta}}           \def\bDelta {\bfsym {\Delta}}
 \def\bfeta{\bfsym {\eta}}              \def\bfEta {\bfsym {\Eta}}
 \def\bmu{\bfsym {\mu}}                 \def\bMu {\bfsym {\Mu}}
 \def\bnu{\bfsym {\nu}}
 \def\btheta{\bfsym {\theta}}           \def\bTheta {\bfsym {\Theta}}
 \def\beps{\bfsym \varepsilon}          \def\bEps{\bfsym{\mathcal E}}
 \def\bepsilon{\bfsym \varepsilon}
 \def\bsigma{\bfsym \sigma}             \def\bSigma{\bfsym \Sigma}
 \def\blambda {\bfsym {\lambda}}        \def\bLambda {\bfsym {\Lambda}}
 \def\bomega {\bfsym {\omega}}          \def\bOmega {\bfsym {\Omega}}
 \def\brho   {\bfsym {\rho}}
 \def\btau{\bfsym {\tau}}
 \def\bxi{\bfsym {\xi}}          \def\bXi{\bfsym {\Xi}}
 \def\bzeta{\bfsym {\zeta}}
 \def\bpi{\bfsym {\pi}}          \def\bPi{\bfsym {\Pi}}
\def\bphi{\bfsym {\phi}}          \def\bPhi{\bfsym {\Phi}}

 %--------------------------------
 %
 %  Hat (boldface) in Greek
 %
  \def\halpha{\hat{\alpha}}              \def\hbalpha{\hat{\bfsym \alpha}}
  \def\hbeta{\hat{\beta}}                \def\hbbeta{\hat{\bfsym \beta}}
  \def\hgamma{\hat{\gamma}}              \def\hgamma{\hat{\bfsym \gamma}}
  \def\hGamma{\hat{ \Gamma}}             \def\hbGamma{\hat{\bfsym \Gamma}}
  \def\hdelta{\hat{\delta}}              \def\hbdelta{\hat{\bfsym {\delta}}}
  \def\hDelta {\hat{\Delta}}             \def\hbDelta{\hat{\bfsym {\Delta}}}
  \def\heta{\hat {\eta}}                 \def\hbfeta {\hat{\bfsym {\eta}}}
  \def\hmu{\hat{\mu}}                    \def\hbmu {\hat{\bfsym {\mu}}}
  \def\hnu{\hat{\nu}}                    \def\hbnu {\hat{\bfsym {\nu}}}
  \def\htheta{\hat {\theta}}             \def\hbtheta {\hat{\bfsym {\theta}}}
  \def\hTheta{\hat {\Theta}}             \def\hbTheta {\hat{\bfsym {\Theta}}}
  \def\hbeps{\hat{\bfsym \varepsilon}}   \def\hbepsilon{\hat{\bfsym \varepsilon}}
  \def\hsigma{\hat{\sigma}}              \def\hbsigma{\hat{\bfsym \sigma}}
  \def\hSigma{\hat{\Sigma}}              \def\hbSigma{\hat{\bfsym \Sigma}}
  \def\hlambda{\hat{\lambda}}            \def\hblambda{\hat{\bfsym \lambda}}
  \def\hLambda{\hat{\Lambda}}            \def\hbLambda{\hat{\bfsym \Lambda}}
  \def\homega {\hat {\omega}}            \def\hbomega {\hat{\bfsym {\omega}}}
  \def\hOmega {\hat {\omega}}            \def\hbOmega {\hat{\bfsym {\Omega}}}
  \def\hrho   {\hat {\rho}}              \def\hbrho {\hat{\bfsym {\rho}}}
  \def\htau   {\hat {\tau}}              \def\hbtau {\hat{\bfsym {\tau}}}
  \def\hxi{\hat{\xi}}                    \def\hbxi{\hat{\bfsym {\xi}}}
  \def\hzeta{\hat{\zeta}}                \def\hbzeta{\hat{\bfsym {\bzeta}}}
\def\eps{\varepsilon}
\def\ve{\varepsilon}
\def\bz{\mathbf z}
\def\bzeta{\bfsym \zeta}
 %--------------------------------
 %
 %  Operator
 %
\providecommand{\abs}[1]{\left\lvert#1\right\rvert}
\providecommand{\norm}[1]{\left\lVert#1\right\rVert}

\providecommand{\angles}[1]{\left\langle #1 \right\rangle}
\providecommand{\paran}[1]{\left( #1 \right)}
\providecommand{\brackets}[1]{\left[ #1 \right]}
\providecommand{\braces}[1]{\left\{ #1 \right\}}

\providecommand{\convprob}{\stackrel{\calP}{\longrightarrow}}
\providecommand{\convdist}{\stackrel{\calD}{\longrightarrow}}
\providecommand{\defeq}{\triangleq}
% \providecommand{\defeq}{\dot{=}}

\usepackage{mathtools}
% K-L divergence
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1 \; \delimsize\| \; #2%
}
\newcommand{\infdiv}{\calD \infdivx}
\newcommand{\kldiv}{\calD_{KL} \infdivx}

%--------------------------------
%
% Regular font in math equation
%

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\corr}{corr}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Dev}{Dev}
\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\E}{E}
\newcommand{\E}[1]{{\mathbb{E}} \left[ #1 \right]}
\DeclareMathOperator{\logit}{logit}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\RSS}{RSS}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\SE}{SE}
%\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
%\DeclareMathOperator{\vect}{vec}
\newcommand{\vect}[1]{{\textsc{Vec}} \left( #1 \right)}
\newcommand{\mat}[1]{{\textsc{Mat}} \left( #1 \right)}


%--------------------------------
%
%  Thms, Props, Assumps, Remarks, et al
%

\newtheorem{definition}{Definition}[section]
\newtheorem{assumption}[definition]{Assumption}
\newtheorem{lemma}[definition]{Lemma}
\newtheorem{proposition}[definition]{Proposition}
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{exercise}[definition]{Exercise}
\newtheorem{example}[definition]{Example}
\newenvironment{solution}{\paragraph{Solution:}}{\hfill$\square$}

\renewcommand*{\theassumption}{\Alph{assumption}}

\def\remark{{\noindent\underbar{\bf Remark}\quad}}

\newenvironment{response}{ \noindent\textit{\textbf{Response: }} \normalfont }{\hfill$\diamondsuit$}
% \color{teal} $\heartsuit$
%--------------------------------
%
%  Bachmann-Landau or asymptotic notations
%
% determiniastic convergence
\newcommand{\bigO}[1]{ \mathcal{O} \left( #1 \right) }
\newcommand{\bigOmega}[1]{ \Omega \left( #1 \right) }
\newcommand{\bigTheta}[1]{ \Theta \left( #1 \right) }
\newcommand{\smlo}[1]{{\rm o} \left( #1 \right) }
\newcommand{\smlomega}[1]{{\omega} \left( #1 \right) }

% converge in probability
\newcommand{\Op}[1]{{\mathcal{O}_p} \left( #1 \right) }
\newcommand{\op}[1]{{\rm o_p} \left( #1 \right) }


%--------------------------------
%
%  Define more colors
%
% need \usepackage[table,xcdraw,dvipsnames]{xcolor}   % for \textcolor
%
%\definecolor{royalpurple}{rgb}{0.47, 0.32, 0.66}
%\definecolor{greenfresh}{HTML}{00897B}
%\definecolor{bluefresh}{HTML}{1E88E5}
%\definecolor{redfresh}{HTML}{E53935}
%--------------------------------
%
%  Markers
%
% need \usepackage[table,xcdraw,dvipsnames]{xcolor}   % for \textcolor

% colorful text emphasizer
\providecommand{\textem}[1]{\textit{\textcolor{Cerulean}{#1}}}

% comments
\providecommand{\elynn}[1]{\textcolor{RubineRed}{\bf [Elynn: #1]}}
\providecommand{\xuening}[1]{\textcolor{blue}{\bf [Xuening: #1]}}

% different attention levels
% a being the most difficult one
\providecommand{\attn}[1]{\textcolor{orange}{\bf (#1)}}
\providecommand{\attna}[1]{\textcolor{redfresh}{\bf (#1)}}
\providecommand{\attnb}[1]{\textcolor{bluefresh}{\bf (#1)}}
\providecommand{\attnc}[1]{\textcolor{greenfresh}{\bf (#1)}}

 %--------------------------------
 %
 %  Shorthands
 %

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}

\def\wt{\widetilde}

\def\blue{\color{blue}}
\def\red{\color{red}}

% May add more in future. 

==> macros/self-defined_v0.tex <==
% Copy right @ 2019
% All right reserved by Elynn Y. Chen.
% This file defines short-hands for math formulas.
% It started with  Prof. Jianqing Fan's macro definition.
% Later it incorporated some of my own macro definition.
%
%
% Other references:
% -- math guide: http://mirrors.rit.edu/CTAN/info/short-math-guide/short-math-guide.pdf
% -- bold math symbol: https://tex.stackexchange.com/questions/595/how-can-i-get-bold-math-symbols
%
%

\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}

%--------------------------------
%
%  Boldfaces in Letters
%
% \newcommand{\bfm}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\bfm}[1]{\ensuremath{\boldsymbol{#1}}} % bm

\def\bzero{\bfm 0}
\def\bone{\bfm 1}
\def\bbone{\mathbbm{1}} % package bm

\def\ba{\bfm a}   \def\bA{\bfm A}  \def\AA{\mathbb{A}}
\def\bb{\bfm b}   \def\bB{\bfm B}  \def\BB{\mathbb{B}}
\def\bc{\bfm c}   \def\bC{\bfm C}  \def\CC{\mathbb{C}}
\def\bd{\bfm d}   \def\bD{\bfm D}  \def\DD{\mathbb{D}}
\def\be{\bfm e}   \def\bE{\bfm E}  \def\EE{\mathbb{E}}
\def\bff{\bfm f}  \def\bF{\bfm F}  \def\FF{\mathbb{F}}
\def\bg{\bfm g}   \def\bG{\bfm G}  \def\GG{\mathbb{G}}
\def\bh{\bfm h}   \def\bH{\bfm H}  \def\HH{\mathbb{H}}
\def\bi{\bfm i}   \def\bI{\bfm I}  \def\II{\mathbb{I}}
\def\bj{\bfm j}   \def\bJ{\bfm J}  \def\JJ{\mathbb{J}}
\def\bk{\bfm k}   \def\bK{\bfm K}  \def\KK{\mathbb{K}}
\def\bl{\bfm l}   \def\bL{\bfm L}  \def\LL{\mathbb{L}}
\def\bm{\bfm m}   \def\bM{\bfm M}  \def\MM{\mathbb{M}}
\def\bn{\bfm n}   \def\bN{\bfm N}  \def\NN{\mathbb{N}}
\def\bo{\bfm o}   \def\bO{\bfm O}  \def\OO{\mathbb{O}}
\def\bp{\bfm p}   \def\bP{\bfm P}  \def\PP{\mathbb{P}}
\def\bq{\bfm q}   \def\bQ{\bfm Q}  \def\QQ{\mathbb{Q}}
\def\br{\bfm r}   \def\bR{\bfm R}  \def\RR{\mathbb{R}}
\def\bs{\bfm s}   \def\bS{\bfm S}  \def\SS{\mathbb{S}}
\def\bt{\bfm t}   \def\bT{\bfm T}  \def\TT{\mathbb{T}}
\def\bu{\bfm u}   \def\bU{\bfm U}  \def\UU{\mathbb{U}}
\def\bv{\bfm v}   \def\bV{\bfm V}  \def\VV{\mathbb{V}}
\def\bw{\bfm w}   \def\bW{\bfm W}  \def\WW{\mathbb{W}}
\def\bx{\bfm x}   \def\bX{\bfm X}  \def\XX{\mathbb{X}}
\def\by{\bfm y}   \def\bY{\bfm Y}  \def\YY{\mathbb{Y}}
\def\bz{\bfm z}   \def\bZ{\bfm Z}  \def\ZZ{\mathbb{Z}}


\def\calA{{\cal  A}} \def\cA{{\cal  A}}
\def\calB{{\cal  B}} \def\cB{{\cal  B}}
\def\calC{{\cal  C}} \def\cC{{\cal  C}}
\def\calD{{\cal  D}} \def\cD{{\cal  D}}
\def\calE{{\cal  E}} \def\cE{{\cal  E}}
\def\calF{{\cal  F}} \def\cF{{\cal  F}}
\def\calG{{\cal  G}} \def\cG{{\cal  G}}
\def\calH{{\cal  H}} \def\cH{{\cal  H}}
\def\calI{{\cal  I}} \def\cI{{\cal  I}}
\def\calJ{{\cal  J}} \def\cJ{{\cal  J}}
\def\calK{{\cal  K}} \def\cK{{\cal  K}}
\def\calL{{\cal  L}} \def\cL{{\cal  L}}
\def\calM{{\cal  M}} \def\cM{{\cal  M}}
\def\calN{{\cal  N}} \def\cN{{\cal  N}}
\def\calO{{\cal  O}} \def\cO{{\cal  O}}
\def\calP{{\cal  P}} \def\cP{{\cal  P}}
\def\calQ{{\cal  Q}} \def\cQ{{\cal  Q}}
\def\calR{{\cal  R}} \def\cR{{\cal  R}}
\def\calS{{\cal  S}} \def\cS{{\cal  S}}
\def\calT{{\cal  T}} \def\cT{{\cal  T}}
\def\calU{{\cal  U}} \def\cU{{\cal  U}}
\def\calV{{\cal  V}} \def\cV{{\cal  V}}
\def\calW{{\cal  W}} \def\cW{{\cal  W}}
\def\calX{{\cal  X}} \def\cX{{\cal  X}}
\def\calY{{\cal  Y}} \def\cY{{\cal  Y}}
\def\calZ{{\cal  Z}} \def\cZ{{\cal  Z}}

%--------------------------------
%
%  Boldfaces in Greek
%
\newcommand{\bfsym}[1]{\ensuremath{\boldsymbol{#1}}}

 \def\balpha{\bfsym \alpha}
 \def\bbeta{\bfsym \beta}
 \def\bgamma{\bfsym \gamma}             \def\bGamma{\bfsym \Gamma}
 \def\bdelta{\bfsym {\delta}}           \def\bDelta {\bfsym {\Delta}}
 \def\bfeta{\bfsym {\eta}}              \def\bfEta {\bfsym {\Eta}}
 \def\bmu{\bfsym {\mu}}                 \def\bMu {\bfsym {\Mu}}
 \def\bnu{\bfsym {\nu}}
 \def\btheta{\bfsym {\theta}}           \def\bTheta {\bfsym {\Theta}}
 \def\beps{\bfsym \varepsilon}          \def\bEps{\bfsym{\mathcal E}}
 \def\bepsilon{\bfsym \varepsilon}
 \def\bve{\bfsym \varepsilon}
 \def\bsigma{\bfsym \sigma}             \def\bSigma{\bfsym \Sigma}
 \def\blambda {\bfsym {\lambda}}        \def\bLambda {\bfsym {\Lambda}}
 \def\bomega {\bfsym {\omega}}          \def\bOmega {\bfsym {\Omega}}
 \def\brho   {\bfsym {\rho}}
 \def\btau{\bfsym {\tau}}
 \def\bxi{\bfsym {\xi}}          \def\bXi{\bfsym {\Xi}}
 \def\bzeta{\bfsym {\zeta}}
 \def\bpi{\bfsym {\pi}}          \def\bPi{\bfsym {\Pi}}
\def\bphi{\bfsym {\phi}}          \def\bPhi{\bfsym {\Phi}}

\def\bLam {\bLambda}
\def\one {\mathbbm{1}}
\def\mR {\mathbb{R}}
\def\cor{\mbox{cor}}
\def\mU{{\mathcal  U}}
 %--------------------------------
 %
 %  Hat (boldface) in Greek
 %
  \def\halpha{\hat{\alpha}}              \def\hbalpha{\hat{\bfsym \alpha}}
  \def\hbeta{\hat{\beta}}                \def\hbbeta{\hat{\bfsym \beta}}
  \def\hgamma{\hat{\gamma}}              \def\hgamma{\hat{\bfsym \gamma}}
  \def\hGamma{\hat{ \Gamma}}             \def\hbGamma{\hat{\bfsym \Gamma}}
  \def\hdelta{\hat{\delta}}              \def\hbdelta{\hat{\bfsym {\delta}}}
  \def\hDelta {\hat{\Delta}}             \def\hbDelta{\hat{\bfsym {\Delta}}}
  \def\heta{\hat {\eta}}                 \def\hbfeta {\hat{\bfsym {\eta}}}
  \def\hmu{\hat{\mu}}                    \def\hbmu {\hat{\bfsym {\mu}}}
  \def\hnu{\hat{\nu}}                    \def\hbnu {\hat{\bfsym {\nu}}}
  \def\htheta{\hat {\theta}}             \def\hbtheta {\hat{\bfsym {\theta}}}
  \def\hTheta{\hat {\Theta}}             \def\hbTheta {\hat{\bfsym {\Theta}}}
  \def\hbeps{\hat{\bfsym \varepsilon}}   \def\hbepsilon{\hat{\bfsym \varepsilon}}
  \def\hsigma{\hat{\sigma}}              \def\hbsigma{\hat{\bfsym \sigma}}
  \def\hSigma{\hat{\Sigma}}              \def\hbSigma{\hat{\bfsym \Sigma}}
  \def\hlambda{\hat{\lambda}}            \def\hblambda{\hat{\bfsym \lambda}}
  \def\hLambda{\hat{\Lambda}}            \def\hbLambda{\hat{\bfsym \Lambda}}
  \def\homega {\hat {\omega}}            \def\hbomega {\hat{\bfsym {\omega}}}
  \def\hOmega {\hat {\omega}}            \def\hbOmega {\hat{\bfsym {\Omega}}}
  \def\hrho   {\hat {\rho}}              \def\hbrho {\hat{\bfsym {\rho}}}
  \def\htau   {\hat {\tau}}              \def\hbtau {\hat{\bfsym {\tau}}}
  \def\hxi{\hat{\xi}}                    \def\hbxi{\hat{\bfsym {\xi}}}
  \def\hzeta{\hat{\zeta}}                \def\hbzeta{\hat{\bfsym {\bzeta}}}
  \def\mE{\mathcal{E}}
  \def\ve{\varepsilon}
  \def\mF{\mathcal{F}}
  \def\mI{{\mathcal  I}}
\def\mG{\mathcal G}
\def\mS{\mathcal S}
\def\mC{\mathcal C}
\def\mV{\mathcal V}


 %--------------------------------
 %
 %  Operator
 %
\providecommand{\abs}[1]{\left\lvert#1\right\rvert}
\providecommand{\norm}[1]{\left\lVert#1\right\rVert}

\providecommand{\angles}[1]{\left\langle #1 \right\rangle}
\providecommand{\paran}[1]{\left( #1 \right)}
\providecommand{\brackets}[1]{\left[ #1 \right]}
\providecommand{\braces}[1]{\left\{ #1 \right\}}

\providecommand{\convprob}{\stackrel{\calP}{\longrightarrow}}
\providecommand{\convdist}{\stackrel{\calD}{\longrightarrow}}
\providecommand{\defeq}{\triangleq}
% \providecommand{\defeq}{\dot{=}}

\usepackage{mathtools}
% K-L divergence
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1 \; \delimsize\| \; #2%
}
\newcommand{\infdiv}{\calD \infdivx}
\newcommand{\kldiv}{\calD_{KL} \infdivx}

%--------------------------------
%
% Regular font in math equation
%

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\corr}{corr}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Dev}{Dev}
\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\E}{E}
\newcommand{\E}[1]{{\mathbb{E}} \left[ #1 \right]}
\DeclareMathOperator{\logit}{logit}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\RSS}{RSS}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\SE}{SE}
%\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
%\DeclareMathOperator{\vect}{vec}
\newcommand{\vect}[1]{{\textsc{Vec}} \left( #1 \right)}
\newcommand{\mat}[1]{{\textsc{Mat}} \left( #1 \right)}


%--------------------------------
%
%  Thms, Props, Assumps, Remarks, et al
%

\newtheorem{definition}{Definition}[section]
\newtheorem{assumption}[definition]{Assumption}
\newtheorem{lemma}[definition]{Lemma}
\newtheorem{proposition}[definition]{Proposition}
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{exercise}[definition]{Exercise}
\newtheorem{example}[definition]{Example}
\newenvironment{solution}{\paragraph{Solution:}}{\hfill$\square$}

\renewcommand*{\theassumption}{\Alph{assumption}}

%\def\remark{{\noindent\underbar{\bf Remark}\quad}}
\theoremstyle{definition}
%\newtheorem*{remark}{\underbar{\bf Remark}}
\newtheorem{remark}{Remark}

\newenvironment{response}{ \textit{\textbf{Response: }} \normalfont }{\hfill$\diamondsuit$}


%--------------------------------
%
%  Bachmann-Landau or asymptotic notations
%
% determiniastic convergence
\newcommand{\bigO}[1]{ \mathcal{O} \left( #1 \right) }
\newcommand{\bigOmega}[1]{ \Omega \left( #1 \right) }
\newcommand{\bigTheta}[1]{ \Theta \left( #1 \right) }
\newcommand{\smlo}[1]{{\rm o} \left( #1 \right) }
\newcommand{\smlomega}[1]{{\omega} \left( #1 \right) }

% converge in probability
\newcommand{\Op}[1]{{\mathcal{O}_p} \left( #1 \right) }
\newcommand{\op}[1]{{\rm o_p} \left( #1 \right) }

%--------------------------------
%
%  Markers
%

% need \usepackage[table,xcdraw,dvipsnames]{xcolor}   % for \textcolor
\definecolor{royalpurple}{rgb}{0.47, 0.32, 0.66}
\providecommand{\elynn}[1]{\textcolor{RubineRed}{\bf [Elynn: #1]}}
\providecommand{\attn}[1]{\textcolor{red}{\bf (#1)}}
\providecommand{\xuening}[1]{\textcolor{blue}{\bf [Xuening: #1]}}

 %--------------------------------
 %
 %  Shorthands
 %

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}

\def\bet{\begin{theorem}}
\def\eet{\end{theorem}}


\def\bel{\begin{lemma}}
\def\eel{\end{lemma}}

\def\eps{\varepsilon}
\def\blam{\blambda}

\def\vec{\mbox{vec}}
\def\wt{\widetilde}
\def\ol{\overline}
\def\wh{\widehat}
\def\blue{\color{blue}}
\def\red{\color{red}}
\def\zero{\mathbf{0}}
\def\tr{\mbox{tr}}

% May add more in future. 
